AdaCCD: Adaptive Semantic Contrasts Discovery Based Cross Lingual Adaptation for Code Clone Detection

Code Clone Detection, which aims to retrieve functionally similar programs from large code bases, has been attracting increasing attention. Modern software often involves a diverse range of programming languages. However, current code clone detection methods are generally limited to only a few popular programming languages due to insufficient annotated data as well as their own model design constraints. To address these issues, we present AdaCCD, a novel cross-lingual adaptation method that can detect cloned codes in a new language without annotations in that language. AdaCCD leverages language-agnostic code representations from pre-trained programming language models and propose an Adaptively Refined Contrastive Learning framework to transfer knowledge from resource-rich languages to resource-poor languages. We evaluate the cross-lingual adaptation results of AdaCCD by constructing a multilingual code clone detection benchmark consisting of 5 programming languages. AdaCCD achieves significant improvements over other baselines, and achieve comparable performance to supervised fine-tuning.

==> components/tables/dataset_statistic.tex <==
\begin{table}[!ht]
    \centering
    \begin{tabular}{cccc}
    \toprule
     Language & Train & Valid & Test  \\
     \midrule
     Ruby & 15345/64 & 3833/16 & 5751/24 \\
     C\# & 17014/160 & 4239/40 & 5280/50 \\
     Rust & 8133/150 & 1334/25 & 1370/25 \\
     JavaScript & 7814/160 & 1904/40 & 2519/50 \\
     Go & 9570/120 & 1595/20 & 1598/20 \\
     \toprule
    \end{tabular}
    \caption{Benchmark Statistics. Number of programs/Number of problems of each language in Train, Valid, and Test splits. Note that the set of problems in Train/Valid/Test splits are disjoint.}
    \label{tb:data-statistics}
\end{table}
